Schema Matching using Machine Learning

Schema Matching is a method of finding attributes that are either similar to each other linguistically or represent the same information. In this project, we take a hybrid approach at solving this problem by making use of both the provided data and the schema name to perform one to one schema matching and introduce the creation of a global dictionary to achieve one to many schema matching. We experiment with two methods of one to one matching and compare both based on their F-scores, precision, and recall. We also compare our method with the ones previously suggested and highlight differences between them.

==> onetomany <==
One to many matching is done when a single attribute in the source schema matches with two or more attributes in the test schema. For example, the address of an individual can either be represented as `Address' in a sigle column or be broken down into `House No' and `Street no\name' as two independent columns. For achieving one to many schema matching, we propose the creation of a global dictionary that contains all possible mappings of a single attribute to multiple attributes and use this as a checkpoint to find out possible one to many mappings. This dictionray is represented as a set of key-value pairs, where keys are those attributes that can be broken down into several smaller ones and values are the corresponding set of attributes that together match with the key. In the example given above, `Address' will be considered a key and `House No' and `Street no\name' will be its corresponding values. Once prepared, this dictionary can be used for 

